Promises and Pitfalls of Threshold-based Auto-labeling

Creating large-scale high-quality labeled datasets is a major bottleneck in supervised machine learning workflows. Threshold-based auto-labeling (TBAL), where validation data obtained from humans is used to find a confidence threshold above which the data is machine-labeled, reduces reliance on manual annotation. TBAL is emerging as a widely-used solution in practice. Given the long shelf-life and diverse usage of the resulting datasets, understanding when the data obtained by such auto-labeling systems can be relied on is crucial. This is the first work to analyze TBAL systems and derive sample complexity bounds on the amount of human-labeled validation data required for guaranteeing the quality of machine-labeled data. Our results provide two crucial insights. First, reasonable chunks of unlabeled data can be automatically and accurately labeled by seemingly bad models. Second, a hidden downside of TBAL systems is potentially prohibitive validation data usage. Together, these insights describe the promise and pitfalls of using such systems. We validate our theoretical guarantees with extensive experiments on synthetic and real datasets.

==> sections/short_related_work.tex <==
\vspace{-5pt}
\section{Related Works}
\label{sec:short_related_works}
%In this section, 
We briefly review related work, deferring a more detailed discussion to the Appendix \ref{sec:extd_related_works}.

There is a rich body of work on active learning (AL) ~\cite{settles2009active, two-faces, hsu2010algorithms,Hanneke2014Book,HCAL2021} focused on learning the best model in a function class with less labeled data than passive learning. Various AL algorithms have been developed and analyzed, e.g., uncertainty sampling \cite{tong2001support, mussmannDataEff}, disagreement region based~\cite{cal94,hanneke2007discoef}, margin based~\cite{balcan2013active} and abstention based methods that minimize the Chow's excess risk~\cite{zhu2022efficient}. 
% It continues to be an active area of research. 

Selective classification (SC) equips a given classifier with the option to abstain from prediction in order to guarantee prediction quality. The foundations for SC are laid down in  \cite{Yaniv2010Selective,wiener2011agnostic, el2012active,wiener2015agnostic} where results on the error rate in the prediction region and the coverage of the given classifier are provided. However, these works lack practical algorithms to find the prediction region. A recent work \cite{gelbhart2019relationship} gives a disagreement-based active learning strategy to learn a selective classifier.    

%A recent work studies a practical algorithm for threshold-based selective classification on deep neural networks \cite{ Yaniv2017Selective}. The algorithm estimates the prediction threshold using training samples and they bound the error rate of the selective classifier using \cite{Gascuel92}. We note that their result is applicable to a specific setting of a given classifier. In contrast, in the TBAL algorithm analyzed in this paper, selective classification is done in each round and the classifiers are not given a priori but instead learned via ERM on training data which is adaptively sampled in each round. 

%typo invented a new word classifiction

A recent paper \cite{qiu2020min-cost-al} studies a TBAL-like algorithm for auto-labeling. It focuses on the cost of training incurred when these systems use large-scale model classes for auto-labeling. It proposes an algorithm to predict the  training set size that minimizes the overall cost and provides an empirical evaluation. 


%We briefly discuss other methods of auto-labeling that do not rely on getting human labels but instead use potentially noisy but cheaply available sources to infer the correct labels \cite{Ratner16, Ratner18, fu2020fast}. While promising, a potential downside is that they can give noisy labels and may not be suitable for high risk applications.
Weak supervision is another line of work aimed at auto-labeling that does not rely on obtaining human labels but instead uses potentially noisy but cheaply available sources to infer labels \cite{Ratner16, fu2020fast}. In contrast, we are focused specifically on analyzing the performance of TBAL algorithms~\cite{sgt}. %The focus of this paper, however, is on analyzing the performance of TBAL algorithms~\cite{sgt} that have emerged recently as auto-labeling solutions in systems. %such as Sagemaker Ground Truth~\cite{sgt}.
%other auto-labeling stuff, weak sup.


==> sections/val_size_vary_figs.tex <==
  \begin{figure*}[t]
  \vspace{-8pt}
  \centering
  \mbox{
  \hspace{-10pt}
    \subfigure[Unit-Ball: with No-UCB ($C_1=0$), $\epsilon_a=1\%$. \label{fig:unit-ball-val-no-ucb}]{\includegraphics[scale=0.285]{figures/v3/unitball_val_eps_0.01_c1_0_nq_500_'lgd_False'.pdf}}
    %{\includegraphics[scale=0.26,trim= 5 37 5 5,clip ]
    \hspace{1pt}
    
    \subfigure[Unit-Ball: with UCB ($C_1=0.25$), $\epsilon_a=1\%$.\label{fig:unit-ball-val-ucb}]{\includegraphics[scale=0.285]{figures/v3/unitball_val_eps_0.01_c1_0.25_nq_500_'lgd_False'.pdf}}
  }

  \mbox{
  \hspace{-12pt}
    \subfigure[ Tiny-Imagenet with No-UCB ($C_1=0$), $\epsilon_a=10\%$ \label{fig:imgnet-val-no-ucb}]{\includegraphics[scale=0.285]{figures/v3/imgnet_val_eps_0.1_c1_0_nq_5000_lgd_True.pdf}}
    \hspace{1pt}
    \subfigure[  Tiny-Imagenet: with UCB ($C_1=0.25$), $\epsilon_a=10\%$ \label{fig:imgnet-val-ucb}]{\includegraphics[scale=0.285]{figures/v3/imgnet_val_eps_0.1_c1_0.25_nq_5000_lgd_True.pdf}}
  }
\vspace{-5pt}
  \caption{ Effect of variation of validation data size with and without using a UCB on error estimates. We keep the maximum number of training samples fixed at 500, 4000, and 5000 for Unit-ball, IMDB, and Tiny-Imagenet respectively.   }
 \vspace{-7pt}
  \label{fig:val_exp_main}
\end{figure*}


==> tables/full_tables/tiny_imgnet_n_v_c1_0.25_n_q_6k_full_tab.tex <==
\begin{table}[t] 
 \scalebox{0.72}{ 
 \begin{tabular}{r|ccccc|ccccc}
\toprule
\multirow{2}{*}{$\mathbf{N_v}$} & \multicolumn{5}{c}{\textbf{Error (\%)} } &  \multicolumn{5}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-11}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{PL+SC}} & {\textbf{AL}} & {\textbf{PL}} & {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{PL+SC}} &{\textbf{AL}} & {\textbf{PL}} \\
\toprule 
2000 & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0}   \\ 
 \midrule 
4000 & 8.08 \tiny{$\pm$0.30} & 4.84 \tiny{$\pm$2.74} & 5.28 \tiny{$\pm$0.36} & 38.71 \tiny{$\pm$0.06} & 33.50 \tiny{$\pm$0.08} & 0.41 \tiny{$\pm$0.03} & 0.42 \tiny{$\pm$0.01} & 0.41 \tiny{$\pm$0.01} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}   \\ 
 \midrule 
6000 & 10.71 \tiny{$\pm$1.28} & 8.68 \tiny{$\pm$1.86} & 8.65 \tiny{$\pm$0.49} & 38.40 \tiny{$\pm$0.36} & 33.50 \tiny{$\pm$0.15} & 8.65 \tiny{$\pm$1.08} & 4.08 \tiny{$\pm$0.28} & 5.83 \tiny{$\pm$1.35} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}   \\ 
 \midrule 
8000 & 9.78 \tiny{$\pm$0.18} & 7.43 \tiny{$\pm$0.81} & 7.87 \tiny{$\pm$0.92} & 38.40 \tiny{$\pm$0.36} & 33.50 \tiny{$\pm$0.15} & 20.93 \tiny{$\pm$1.07} & 12.29 \tiny{$\pm$1.41} & 17.90 \tiny{$\pm$1.11} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}   \\ 
 \midrule 
10000 & 9.27 \tiny{$\pm$0.32} & 7.30 \tiny{$\pm$0.29} & 7.42 \tiny{$\pm$0.43} & 38.40 \tiny{$\pm$0.36} & 33.50 \tiny{$\pm$0.15} & 29.29 \tiny{$\pm$0.53} & 17.93 \tiny{$\pm$0.96} & 25.37 \tiny{$\pm$0.59} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}\\ 
 \toprule 
 \end{tabular}
 } 
  \caption{Tiny-Imagenet, $C_1=0.25$, $N_q=6K, \epsilon_a=10\%$}
 \end{table}

==> tables/full_tables/tiny_imgnet_n_v_c1_0_n_q_6k_full_tab.tex <==
\begin{table}[t] 
 \scalebox{0.72}{ 
 \begin{tabular}{r|ccccc|ccccc}
\toprule
\multirow{2}{*}{$\mathbf{N_v}$} & \multicolumn{5}{c}{\textbf{Error (\%)} } &  \multicolumn{5}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-11}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{PL+SC}} & {\textbf{AL}} & {\textbf{PL}} & {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{PL+SC}} &{\textbf{AL}} & {\textbf{PL}} \\
\toprule 
2000 & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0}   \\ 
 \midrule 
4000 & 17.60 \tiny{$\pm$6.27} & 4.84 \tiny{$\pm$2.74} & 17.76 \tiny{$\pm$4.87} & 38.71 \tiny{$\pm$0.06} & 33.45 \tiny{$\pm$0.11} & 0.71 \tiny{$\pm$0.33} & 0.42 \tiny{$\pm$0.01} & 0.49 \tiny{$\pm$0.03} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}   \\ 
 \midrule 
6000 & 15.11 \tiny{$\pm$0.94} & 10.94 \tiny{$\pm$1.17} & 12.90 \tiny{$\pm$0.58} & 38.40 \tiny{$\pm$0.36} & 33.50 \tiny{$\pm$0.15} & 14.29 \tiny{$\pm$1.17} & 6.52 \tiny{$\pm$1.35} & 10.84 \tiny{$\pm$0.84} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}   \\ 
 \midrule 
8000 & 14.22 \tiny{$\pm$0.56} & 11.65 \tiny{$\pm$0.40} & 12.58 \tiny{$\pm$0.36} & 38.40 \tiny{$\pm$0.36} & 33.50 \tiny{$\pm$0.15} & 31.92 \tiny{$\pm$2.24} & 19.28 \tiny{$\pm$1.16} & 28.89 \tiny{$\pm$1.19} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}   \\ 
 \midrule 
10000 & 13.71 \tiny{$\pm$0.36} & 11.65 \tiny{$\pm$0.36} & 12.24 \tiny{$\pm$0.12} & 38.40 \tiny{$\pm$0.36} & 33.50 \tiny{$\pm$0.15} & 38.57 \tiny{$\pm$1.06} & 28.13 \tiny{$\pm$0.39} & 37.90 \tiny{$\pm$1.05} & 97.00 \tiny{$\pm$0.00} & 94.00 \tiny{$\pm$0.00}\\ 
 \toprule 
 \end{tabular}
 }
 \caption{Tiny-Imagenet, $C_1=0$, $N_q=6K, \epsilon_a=10\%$}
 \end{table}

==> tables/small_tables/imdb-table-c1_0.25.tex <==


\begin{table}[h]
\hspace{-10pt}
\begin{tabular}{r|ll|ll}
\toprule
 \multirow{2}{*}{N\_b} &

      \multicolumn{2}{c}{Error (\%)} &
      \multicolumn{2}{c}{Coverage (\%)} \\
     
      & {TBAL} & {AL+SC} & {TBAL} & {AL+SC}  \\
      
\midrule
300 & 1.82 \tiny{$\pm$0.07} & 1.88 \tiny{$\pm$0.29} & 76.97 \tiny{$\pm$1.18} & 61.84 \tiny{$\pm$15.52}   \\ 
400 & 1.79 \tiny{$\pm$0.15} & 1.74 \tiny{$\pm$0.28} & 76.90 \tiny{$\pm$2.37} & 68.12 \tiny{$\pm$16.52}   \\ 
500 & 1.95 \tiny{$\pm$0.25} & 2.00 \tiny{$\pm$0.28} & 76.51 \tiny{$\pm$3.48} & 70.71 \tiny{$\pm$4.43}   \\ 
600 & 1.93 \tiny{$\pm$0.09} & 1.92 \tiny{$\pm$0.24} & 76.17 \tiny{$\pm$3.49} & 73.44 \tiny{$\pm$3.39}   \\ 
700 & 1.79 \tiny{$\pm$0.15} & 1.95 \tiny{$\pm$0.35} & 76.37 \tiny{$\pm$2.61} & 72.40 \tiny{$\pm$8.55}   \\ 
800 & 1.84 \tiny{$\pm$0.12} & 1.96 \tiny{$\pm$0.23} & 77.50 \tiny{$\pm$2.24} & 70.00 \tiny{$\pm$10.92}   \\ 
900 & 1.97 \tiny{$\pm$0.12} & 2.02 \tiny{$\pm$0.16} & 77.78 \tiny{$\pm$2.62} & 74.19 \tiny{$\pm$6.70}   \\ 

\bottomrule
\end{tabular}
\begin{tabular}{r|ll|ll}
\toprule
 \multirow{2}{*}{N\_v} &

      \multicolumn{2}{c}{Error (\%)} &
      \multicolumn{2}{c}{Coverage (\%)} \\
     
      & {TBAL} & {AL+SC} & {TBAL} & {AL+SC}  \\
      
\midrule
100 & 3.10 \tiny{$\pm$1.80} & 0.68 \tiny{$\pm$0.81} & 71.43 \tiny{$\pm$8.86} & 96.95 \tiny{$\pm$1.01}   \\ 
400 & 1.65 \tiny{$\pm$0.65} & 0.32 \tiny{$\pm$0.15} & 93.27 \tiny{$\pm$2.50} & 96.91 \tiny{$\pm$0.99}   \\ 
800 & 1.08 \tiny{$\pm$0.47} & 0.24 \tiny{$\pm$0.16} & 96.01 \tiny{$\pm$1.16} & 96.31 \tiny{$\pm$1.36}   \\ 
1200 & 0.78 \tiny{$\pm$0.27} & 0.17 \tiny{$\pm$0.11} & 96.82 \tiny{$\pm$0.84} & 95.96 \tiny{$\pm$1.40}   \\ 
1600 & 0.65 \tiny{$\pm$0.20} & 0.13 \tiny{$\pm$0.08} & 96.92 \tiny{$\pm$0.57} & 95.70 \tiny{$\pm$1.38}   \\ 
2000 & 0.54 \tiny{$\pm$0.16} & 0.21 \tiny{$\pm$0.11} & 97.23 \tiny{$\pm$0.42} & 96.36 \tiny{$\pm$1.13}   \\ 
2400 & 0.49 \tiny{$\pm$0.14} & 0.18 \tiny{$\pm$0.09} & 97.39 \tiny{$\pm$0.35} & 96.19 \tiny{$\pm$1.21}   \\ 
2800 & 0.45 \tiny{$\pm$0.15} & 0.15 \tiny{$\pm$0.08} & 97.42 \tiny{$\pm$0.29} & 96.09 \tiny{$\pm$1.13}   \\

\bottomrule

\end{tabular}
\caption{ Unit Ball:}
\end{table}

==> tables/small_tables/imdb-table_c1_0.tex <==

\begin{table}[t]
\hspace{-10pt}
\scalebox{0.75} {
\centering
\input{tables/unit_ball_val_c1_0.25_small_tab}
}
\hspace{20pt}
\scalebox{0.8}{
\centering
\begin{tabular}{r|ll|ll}
\toprule
 \multirow{2}{*}{$N_v$} &

      \multicolumn{2}{c}{Error (\%)} &
      \multicolumn{2}{c}{Coverage (\%)} \\
     \midrule
      & {TBAL} & {AL+SC} & {TBAL} & {AL+SC}  \\
      
\midrule
200 & 4.77 \tiny{$\pm$0.18} & 3.35 \tiny{$\pm$0.80} & 83.14 \tiny{$\pm$3.65} & 78.53 \tiny{$\pm$7.05}   \\ 
300 & 4.71 \tiny{$\pm$0.22} & 3.36 \tiny{$\pm$0.81} & 86.08 \tiny{$\pm$4.14} & 79.26 \tiny{$\pm$8.78}   \\ 
400 & 4.57 \tiny{$\pm$0.26} & 3.53 \tiny{$\pm$0.73} & 90.70 \tiny{$\pm$3.11} & 86.39 \tiny{$\pm$5.11}   \\ 
500 & 4.45 \tiny{$\pm$0.23} & 3.80 \tiny{$\pm$0.72} & 92.58 \tiny{$\pm$1.84} & 88.84 \tiny{$\pm$5.21}   \\ 
600 & 4.32 \tiny{$\pm$0.17} & 3.70 \tiny{$\pm$0.63} & 92.96 \tiny{$\pm$0.46} & 88.90 \tiny{$\pm$4.83}   \\ 
700 & 4.63 \tiny{$\pm$0.11} & 3.96 \tiny{$\pm$0.69} & 93.33 \tiny{$\pm$0.19} & 90.49 \tiny{$\pm$3.69}   \\ 
800 & 4.66 \tiny{$\pm$0.20} & 3.84 \tiny{$\pm$0.70} & 92.42 \tiny{$\pm$0.89} & 88.67 \tiny{$\pm$3.88}   \\

\toprule

\end{tabular}
}
\caption{\small{Detailed numbers for selected methods for the IMDB experiment with better feature extraction. Here $N_b$ stands for max no. of training samples the algorithms are allowed to use and  $N_v$ stands for the validation data size. We keep $C_1=0$ for this experiment.}}
\end{table} 

\input{tables/unit_ball_table_val_small}

==> tables/small_tables/imdb_n_q_c1_0_n_v_1000_small_tab.tex <==
\begin{tabular}{r|cc|cc}
\toprule
\multirow{2}{*}{$\mathbf{N_q}$} & \multicolumn{2}{c}{\textbf{Error (\%)} } &  \multicolumn{2}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-5}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{TBAL}} & {\textbf{AL+SC}}  \\
\toprule 
200 & 4.57 \tiny{$\pm$0.21} & 4.30 \tiny{$\pm$0.20} & 93.46 \tiny{$\pm$1.01} & 90.60 \tiny{$\pm$2.91}   \\ 
 \midrule 
400 & 4.60 \tiny{$\pm$0.09} & 3.75 \tiny{$\pm$0.83} & 92.55 \tiny{$\pm$0.66} & 84.27 \tiny{$\pm$19.15}   \\ 
 \midrule 
600 & 4.93 \tiny{$\pm$0.10} & 3.99 \tiny{$\pm$0.91} & 92.45 \tiny{$\pm$0.84} & 91.69 \tiny{$\pm$3.99}   \\ 
 \midrule 
800 & 4.76 \tiny{$\pm$0.12} & 3.55 \tiny{$\pm$0.69} & 92.15 \tiny{$\pm$1.05} & 89.98 \tiny{$\pm$3.38}   \\ 
 \midrule 
1000 & 4.49 \tiny{$\pm$0.06} & 4.19 \tiny{$\pm$0.31} & 92.25 \tiny{$\pm$0.96} & 92.28 \tiny{$\pm$2.13}\\ 
 \toprule 
 \end{tabular}

==> tables/small_tables/tiny_imgnet_n_q_c1_0_n_v_10k_small_tab.tex <==
\begin{tabular}{r|cc|cc}
\toprule
\multirow{2}{*}{$\mathbf{N_q}$} & \multicolumn{2}{c}{\textbf{Error (\%)} } &  \multicolumn{2}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-5}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{TBAL}} & {\textbf{AL+SC}}  \\
\toprule 
2000 & 14.02 \tiny{$\pm$0.26} & 11.49 \tiny{$\pm$0.80} & 24.34 \tiny{$\pm$0.86} & 14.41 \tiny{$\pm$1.00}   \\ 
 \midrule 
4000 & 14.10 \tiny{$\pm$0.77} & 11.58 \tiny{$\pm$0.26} & 34.16 \tiny{$\pm$1.00} & 21.84 \tiny{$\pm$1.36}   \\ 
 \midrule 
6000 & 13.55 \tiny{$\pm$0.17} & 11.33 \tiny{$\pm$0.35} & 37.80 \tiny{$\pm$1.05} & 28.59 \tiny{$\pm$1.53}   \\ 
 \midrule 
8000 & 13.79 \tiny{$\pm$0.27} & 11.72 \tiny{$\pm$0.32} & 42.00 \tiny{$\pm$1.71} & 32.00 \tiny{$\pm$1.12}   \\ 
 \midrule 
10000 & 13.26 \tiny{$\pm$0.35} & 11.42 \tiny{$\pm$0.28} & 43.63 \tiny{$\pm$0.38} & 33.80 \tiny{$\pm$0.82}\\ 
 \toprule 
 \end{tabular}

==> tables/small_tables/tiny_imgnet_val_c1_0.25_n_q_6k_small_tab.tex <==
\begin{tabular}{r|cc|cc}
\toprule
\multirow{2}{*}{$\mathbf{N_v}$} & \multicolumn{2}{c}{\textbf{Error (\%)} } &  \multicolumn{2}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-5}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{TBAL}} & {\textbf{AL+SC}}  \\
\toprule 
2000 & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0}   \\ 
 \midrule 
4000 & 8.08 \tiny{$\pm$0.30} & 4.84 \tiny{$\pm$2.74} & 0.41 \tiny{$\pm$0.03} & 0.42 \tiny{$\pm$0.01}   \\ 
 \midrule 
6000 & 10.71 \tiny{$\pm$1.28} & 8.68 \tiny{$\pm$1.86} & 8.65 \tiny{$\pm$1.08} & 4.08 \tiny{$\pm$0.28}   \\ 
 \midrule 
8000 & 9.78 \tiny{$\pm$0.18} & 7.43 \tiny{$\pm$0.81} & 20.93 \tiny{$\pm$1.07} & 12.29 \tiny{$\pm$1.41}   \\ 
 \midrule 
10000 & 9.27 \tiny{$\pm$0.32} & 7.30 \tiny{$\pm$0.29} & 29.29 \tiny{$\pm$0.53} & 17.93 \tiny{$\pm$0.96}\\ 
 \toprule 
 \end{tabular}

==> tables/small_tables/tiny_imgnet_val_c1_0_n_q_6k_small_tab.tex <==
\begin{tabular}{r|cc|cc}
\toprule
\multirow{2}{*}{$\mathbf{N_v}$} & \multicolumn{2}{c}{\textbf{Error (\%)} } &  \multicolumn{2}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-5}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{TBAL}} & {\textbf{AL+SC}}  \\
\toprule 
2000 & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0} & 0.0 \tiny{$\pm$0.0}   \\ 
 \midrule 
4000 & 17.60 \tiny{$\pm$6.27} & 4.84 \tiny{$\pm$2.74} & 0.71 \tiny{$\pm$0.33} & 0.42 \tiny{$\pm$0.01}   \\ 
 \midrule 
6000 & 15.11 \tiny{$\pm$0.94} & 10.94 \tiny{$\pm$1.17} & 14.29 \tiny{$\pm$1.17} & 6.52 \tiny{$\pm$1.35}   \\ 
 \midrule 
8000 & 14.22 \tiny{$\pm$0.56} & 11.65 \tiny{$\pm$0.40} & 31.92 \tiny{$\pm$2.24} & 19.28 \tiny{$\pm$1.16}   \\ 
 \midrule 
10000 & 13.71 \tiny{$\pm$0.36} & 11.65 \tiny{$\pm$0.36} & 38.57 \tiny{$\pm$1.06} & 28.13 \tiny{$\pm$0.39}\\ 
 \toprule 
 \end{tabular}

==> tables/small_tables/unit-ball_table.tex <==


\begin{table}[h]
\hspace{-10pt}
\begin{tabular}{r|ll|ll}
\toprule
 \multirow{2}{*}{N\_b} &

      \multicolumn{2}{c}{Error (\%)} &
      \multicolumn{2}{c}{Coverage (\%)} \\
     
      & {TBAL} & {AL+SC} & {TBAL} & {AL+SC}  \\
      
\midrule
100 & 0.78 \tiny{$\pm$0.19} & 0.29 \tiny{$\pm$0.25} & 71.40 \tiny{$\pm$5.64} & 19.31 \tiny{$\pm$8.77}   \\ 
200 & 0.49 \tiny{$\pm$0.13} & 0.16 \tiny{$\pm$0.09} & 95.28 \tiny{$\pm$1.29} & 59.41 \tiny{$\pm$10.32}   \\ 
300 & 0.45 \tiny{$\pm$0.11} & 0.16 \tiny{$\pm$0.07} & 97.74 \tiny{$\pm$0.30} & 82.30 \tiny{$\pm$5.40}   \\ 
400 & 0.40 \tiny{$\pm$0.12} & 0.15 \tiny{$\pm$0.07} & 97.63 \tiny{$\pm$0.24} & 92.06 \tiny{$\pm$2.63}   \\ 
500 & 0.37 \tiny{$\pm$0.13} & 0.16 \tiny{$\pm$0.09} & 97.52 \tiny{$\pm$0.18} & 96.22 \tiny{$\pm$0.99}   \\ 
600 & 0.34 \tiny{$\pm$0.13} & 0.12 \tiny{$\pm$0.05} & 97.36 \tiny{$\pm$0.20} & 97.07 \tiny{$\pm$0.57}   \\ 
800 & 0.28 \tiny{$\pm$0.10} & 0.07 \tiny{$\pm$0.03} & 97.10 \tiny{$\pm$0.23} & 97.36 \tiny{$\pm$0.11}   \\ 
1000 & 0.25 \tiny{$\pm$0.10} & 0.03 \tiny{$\pm$0.02} & 96.90 \tiny{$\pm$0.21} & 96.84 \tiny{$\pm$0.03}   \\ 

\bottomrule
\end{tabular}
\begin{tabular}{r|ll|ll}
\toprule
 \multirow{2}{*}{N\_v} &

      \multicolumn{2}{c}{Error (\%)} &
      \multicolumn{2}{c}{Coverage (\%)} \\
     
      & {TBAL} & {AL+SC} & {TBAL} & {AL+SC}  \\
      
\midrule
100 & 3.10 \tiny{$\pm$1.80} & 0.68 \tiny{$\pm$0.81} & 71.43 \tiny{$\pm$8.86} & 96.95 \tiny{$\pm$1.01}   \\ 
400 & 1.65 \tiny{$\pm$0.65} & 0.32 \tiny{$\pm$0.15} & 93.27 \tiny{$\pm$2.50} & 96.91 \tiny{$\pm$0.99}   \\ 
800 & 1.08 \tiny{$\pm$0.47} & 0.24 \tiny{$\pm$0.16} & 96.01 \tiny{$\pm$1.16} & 96.31 \tiny{$\pm$1.36}   \\ 
1200 & 0.78 \tiny{$\pm$0.27} & 0.17 \tiny{$\pm$0.11} & 96.82 \tiny{$\pm$0.84} & 95.96 \tiny{$\pm$1.40}   \\ 
1600 & 0.65 \tiny{$\pm$0.20} & 0.13 \tiny{$\pm$0.08} & 96.92 \tiny{$\pm$0.57} & 95.70 \tiny{$\pm$1.38}   \\ 
2000 & 0.54 \tiny{$\pm$0.16} & 0.21 \tiny{$\pm$0.11} & 97.23 \tiny{$\pm$0.42} & 96.36 \tiny{$\pm$1.13}   \\ 
2400 & 0.49 \tiny{$\pm$0.14} & 0.18 \tiny{$\pm$0.09} & 97.39 \tiny{$\pm$0.35} & 96.19 \tiny{$\pm$1.21}   \\ 
2800 & 0.45 \tiny{$\pm$0.15} & 0.15 \tiny{$\pm$0.08} & 97.42 \tiny{$\pm$0.29} & 96.09 \tiny{$\pm$1.13}   \\

\bottomrule

\end{tabular}
\caption{\small{Detailed numbers for selected methods for the Unit-Ball experiment in the paper. The left table is for Figure 4(a) in the main paper and the right table is for figure 3(b). Here $N_b$ stands for max no. of training samples the algorithms are allowed to use and  $N_v$ stands for the validation data size.} }
\end{table}

==> tables/small_tables/unit_ball_n_q_c1_0.25_small_tab.tex <==
\begin{tabular}{r|cc|cc}
\toprule
\multirow{2}{*}{$\mathbf{N_q}$} & \multicolumn{2}{c}{\textbf{Error (\%)} } &  \multicolumn{2}{c}{\textbf{Coverage (\%)}} \\ 
\cmidrule{2-5}
& {\textbf{TBAL}} & {\textbf{AL+SC}} & {\textbf{TBAL}} & {\textbf{AL+SC}}  \\
\toprule 
100 & 0.78 \tiny{$\pm$0.19} & 0.29 \tiny{$\pm$0.25} & 71.40 \tiny{$\pm$5.64} & 19.31 \tiny{$\pm$8.77}   \\ 
 \midrule 
200 & 0.49 \tiny{$\pm$0.13} & 0.16 \tiny{$\pm$0.09} & 95.28 \tiny{$\pm$1.29} & 59.41 \tiny{$\pm$10.32}   \\ 
 \midrule 
400 & 0.40 \tiny{$\pm$0.12} & 0.15 \tiny{$\pm$0.07} & 97.63 \tiny{$\pm$0.24} & 92.06 \tiny{$\pm$2.63}   \\ 
 \midrule 
600 & 0.34 \tiny{$\pm$0.13} & 0.12 \tiny{$\pm$0.05} & 97.36 \tiny{$\pm$0.20} & 97.07 \tiny{$\pm$0.57}   \\ 
 \midrule 
800 & 0.28 \tiny{$\pm$0.10} & 0.07 \tiny{$\pm$0.03} & 97.10 \tiny{$\pm$0.23} & 97.36 \tiny{$\pm$0.11}   \\ 
 \midrule 
1000 & 0.25 \tiny{$\pm$0.10} & 0.03 \tiny{$\pm$0.02} & 96.90 \tiny{$\pm$0.21} & 96.84 \tiny{$\pm$0.03}\\ 
 \toprule 
 \end{tabular}
